A Nice Labelling for Tree-Like Event Structures of Degree 3

We address the problem of &#64257;nding nice labellings for event structures of degree 3. We develop a minimum theory by which we prove that the labelling number of an event structure of degree 3 is bounded by a linear function of the height. The main theorem we present in this paper states that event structures of degree 3 whose causality order is a tree have a nice labelling with 3 colors. Finally, we exemplify how to use this theorem to construct upper bounds for the labelling number of other event structures of degree 3.

==> macros.tex <==
\RequirePackage{ifthen}

\newcommand{\breath}{\vskip 6pt}
\newcommand{\takebreath}{\vskip -4pt}

\newcommand{\eproofofclaim}{\hfill\mbox{$\Box$\hspace{2mm}\emph{Claim}}\par\breath}

\newenvironment{tbs}{%
   \renewcommand{\labelitemi}{$\blacktriangleright$}%
   \begin{itemize}\tt }{\end{itemize}}
\newcommand{\btbs}{\begin{tbs}}                                         
\begin{draftversion}
  \newcommand{\shtbs}[1]{\begin{tbs} \item #1 \end{tbs}}
\end{draftversion}
\begin{finalversion}
  \newcommand{\shtbs}[1]{}
\end{finalversion}


%%
\newcommand{\myhfill}{\mbox{\hspace{0mm}}\hfill\mbox{\hspace{0mm}}}
\newlength{\mylength}
\newlength{\mylengthu}
\newlength{\mylengthd}
% \newcommand{\overwrite}[2]{%
% \settowidth{\mylength}{\mbox{$#1$}}%
% #1\hspace{-\mylength}#2%
% }
\newcommand{\overwrite}[2]{%
\settowidth{\mylengthu}{\mbox{$#1$}}%
\settowidth{\mylengthd}{\mbox{$#2$}}%
\ifthenelse{\lengthtest{\mylengthu >\mylengthd}}%
{#1\hspace{-\mylengthu}\parbox{\mylengthu}{\myhfill$#2$\myhfill}}%
{#2\hspace{-\mylengthd}\parbox{\mylengthd}{\myhfill$#1$\myhfill}}%
}


%% General
\newcommand{\set}[1]{\{\,#1\,\}}
\newcommand{\couple}[1]{\{#1\}}
%\newcommand{\card}[1]{|#1|}
\newcommand{\card}[1]{\mathrm{card}#1}
\newcommand{\N}{\mathbb{N}}
\newcommand{\quotient}{/\!\!}
\newcommand{\mymod}{\,\mathrm{mod}\,}

%% Particular
\newcommand{\CYf}{\mathcal{SC}_{\geq 4}}

%% Graphs
\newcommand{\cl}{\chi}
\newcommand{\chr}{\gamma}
\newcommand{\nl}{\mathrm{nl}}
\newcommand{\CL}{\mathcal{CL}}

%% Order
\newcommand{\filter}[1]{\uparrow\!\{\,#1\,\}}
\newcommand{\ideal}[1]{\downarrow\!\{\,#1\,\}}
\newcommand{\idealof}[1]{\downarrow\!#1}

\newcommand{\lcover}{\prec}
\newcommand{\lcovers}{\lcover}
\newcommand{\comp}{\simeq}
%\newcommand{\comp}{\overwrite{\leq}{\geq}}
\newcommand{\uncomp}{\not\comp}
\newcommand{\ncomp}{\not\comp}

%\newcommand{\height}{\mathrm{height}}
% \newcommand{\height}[1][]{\hbar_{#1}}
% \newcommand{\width}[1][]{\mathrm{width}}
% \newcommand{\fat}{\mathrm{fat}}
\newcommand{\height}[1][]{\mathrm{h}_{#1}}
\newcommand{\width}[1][]{\mathrm{w}}
\newcommand{\fat}{\mathrm{f}}

\newcommand{\heightp}[1][]{\height[#1]^{\!\!+}}

\newcommand{\depends}{<<}
\newcommand{\compares}{\ll}
%%\newcommand{\lord}{\lessdot}
\newcommand{\lord}{\lhd}
\newcommand{\lc}[1]{lc(#1)}


%%
%% Event structures
%%

\newcommand{\E}{\mathcal{E}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\G}{\mathcal{G}}

\newcommand{\conflict}{\raisebox{-1pt}{$\smile$}}
\newcommand{\confl}{\conflict}
\newcommand{\mytire}{\raisebox{1pt}{$\overline{\hspace{10pt}}$}}
\newcommand{\minimalconflict}{%
  \,%
  \overwrite{\raisebox{1pt}{$\mytire$}}%
  {\raisebox{-1pt}{$\mytire$}}%
  \,%
}
\newcommand{\mconfl}{\minimalconflict}

\newcommand{\concurrent}{\raisebox{2pt}{$\frown$}}
\newcommand{\conc}{\concurrent}
\newcommand{\nconc}{\overwrite{\conc}{/}}

\newcommand{\weakconcurrent}{\overwrite{\concurrent}{\raisebox{-7pt}{$\comp$}}}
\newcommand{\wconc}{\weakconcurrent}

%\newcommand{\orthogonal}{\perp}
\newcommand{\orthogonal}[1][\frown]{{\,\raisebox{-1pt}{$\overline{#1}$}\,}}
%\newcommand{\orthogonal}{\overwrite{\mconfl}{\frown}}
\newcommand{\orth}{\orthogonal}
\newcommand{\north}{\overwrite{\orth}{/}}

\newcommand{\orthogonalp}{\bowtie^{+}}

\newcommand{\directed}{\rightarrow}
\newcommand{\directedb}{\leftarrow}
\newcommand{\CNF}{\mathcal{C}}

\newcommand{\skewn}[1][]{\mathrm{skew}_{#1}}

\newcommand{\Ld}{\mathcal{L}_{0,2}}
\newcommand{\Lu}{\mathcal{L}_{1}}

%%% Logics
\newcommand{\tand}{\textrm{ and }}
\newcommand{\timplies}{\textrm{ implies }}
\newcommand{\tst}{\textrm{ s.t. }}

%% Arrows
\newcommand{\rTo}{\longrightarrow}
\renewcommand{\O}[1][\!\!\lord]{O_{{\!}_{#1}}\!}
\renewcommand{\L}[1][\!\lord]{L_{{\!}_{#1}}\!}
\newcommand{\C}[1][\!\!\lord]{C_{{\!}_{#1}}\!}


%%% XY-pic

\newgraphescape{G}{
  []="q"
  ([r(1.5)]="qa"
  ([u]="qac",[r(1)u(0.5)]="qab"
  [u]="qabc"),
  [r(1)u(0.5)]="qb"
  [u]="qbc",
  [u]="qc")
}

\newgraphescape{d}#1#2{
  []:@{{}{-}{>}}"#1"*+{#1}="#1"^{#2}"#1"
}

\newgraphescape{e}#1#2#3{
  "#1"*+{#1}="#1":"#2"*+{#2}="#2"^{#3}"#2"
}
\newcommand{\cubes}{%
%%
\xymatrix{
  \xybox{%
    \xygraph{
      []!G
      %% AC face
      !e{q}{qa}{a}!e{qa}{qac}{c}
      !e{q}{qc}{c}!e{qc}{qac}{a}
      %% BC face
      !e{qa}{qab}{b}!e{qab}{qabc}{c}
      !e{qac}{qabc}{b}
      %% AB face
      !e{qc}{qbc}{b}!e{qbc}{qabc}{a}
    }
  }
  &
  \Longleftrightarrow
  &
  \xybox{%
    \xygraph{
      []!G
      %% AB face
      !e{q}{qa}{a}
      !e{qa}{qab}{b}
      !e{q}{qb}{b}!e{qb}{qab}{a}
      %% BC face
      !e{qb}{qbc}{c}
      !e{q}{qc}{c}!e{qc}{qbc}{b}
      %% BAC face
      !e{qb}{qab}{a}!e{qab}{qabc}{c}
      !e{qbc}{qabc}{a}
    }
  }
}
%%
}


\newcommand{\coherent}{%
  \xymatrix{
    \xybox{%
      \xygraph{
        []!G
        %% AC face
        !e{q}{qa}{a}!e{qa}{qac}{c}
        !e{q}{qc}{c}!e{qc}{qac}{a}
        %% BC face
        !e{q}{qb}{b}!e{qb}{qbc}{c}
        !e{qc}{qbc}{b}
        %% AB face
        !e{qa}{qab}{b}
        !e{qb}{qab}{a}
      }
    }
    &
    %% \!\!\!\!  
    \Longrightarrow
    %% \!\!\!\!
    &
    \xybox{%
      \xygraph{
        []!G
        %% CAB face
        !e{qc}{qac}{a}
        !e{qac}{qabc}{b}
        !e{qc}{qbc}{b}
        !e{qbc}{qabc}{a}
        %% ABC face
        !e{qa}{qab}{b}
        !e{qab}{qabc}{c}
        !e{qa}{qac}{c}!e{qac}{qabc}{b}
        %% BAC face
        !e{qb}{qab}{a}
        !e{qb}{qbc}{c}
        !e{qab}{qabc}{c}
        !e{qbc}{qabc}{a}
      }
    }
  }
}

\newcommand{\Gzero}{%
  \xygraph{%
    []*+{v_{0}}
  }
}

\newcommand{\Gone}{%
  \xygraph{%
    []*+{v_{1}}
    [r]*+{\tilde{v}_{1}}
  }
}

\newcommand{\Gtwo}{%
  \xygraph{%
    []*+{v_{2}}
    (-[dl]*+{v_{1}},-[dr]*+{\tilde{v}_{1}})
  }
}

\newcommand{\Gthree}{%
  \xygraph{%
    []*+{v_{3}}="S"
    (-[dl]*+{v_{1}}="A",-[dr]*+{\tilde{v}_{1}}="B",
    [dd]*+{\tilde{v}_{3}}="C"
    )
    "C"(-"A",-"B")
  }
}

\newcommand{\Gfour}{$\xygraph{%
    []*+{v_{3}}="S"
    (-[dl]*+{v_{1}}="A",-[dr]*+{\tilde{v}_{1}}="B",
    [dd]*+{\tilde{v}_{3}}="C"
    ,
    "C"(-"A",-"B")
    )
    [u(0.5)ll]*+{v_{4}}
    (-"S",-"A",-@/^9mm/"B",-@/_7mm/"C")
  }$
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 

